Aviary: training language agents on challenging scientific tasks

Solving complex real-world tasks requires cycles of actions and observations. This is particularly true in science, where tasks require many cycles of analysis, tool use, and experimentation. Language agents are promising for automating intellectual tasks in science because they can interact with tools via natural language or code. Yet their flexibility creates conceptual and practical challenges for software implementations, since agents may comprise non-standard components such as internal reasoning, planning, tool usage, as well as the inherent stochasticity of temperature-sampled language models. Here, we introduce Aviary, an extensible gymnasium for language agents. We formalize agents as policies solving language-grounded partially observable Markov decision processes, which we term language decision processes. We then implement five environments, including three challenging scientific environments: (1) manipulating DNA constructs for molecular cloning, (2) answering research questions by accessing scientific literature, and (3) engineering protein stability. These environments were selected for their focus on multi-step reasoning and their relevance to contemporary biology research. Finally, with online training and scaling inference-time compute, we show that language agents backed by open-source, non-frontier LLMs can match and exceed both frontier LLM agents and human experts on multiple tasks at up to 100x lower inference cost.

==> support_information/tools_cloning.tex <==
\subsection{Cloning tools}

\textbf{design\_primers:}
\begin{itemize}
    \item Purpose:
    \begin{itemize}
        \item Creates PCR primers with optional overhangs and a specified melting temperature (Tm) for a given DNA sequence.
    \end{itemize}
    \item Parameters:
    \begin{itemize}
        \item \texttt{sequence}: The DNA sequence to design primers for.
        \item \texttt{forward\_overhang}: Optional extra sequence to add to the forward primer.
        \item \texttt{forward\_overhang\_name}: Optional name of an enzyme to create a matching forward overhang.
        \item \texttt{reverse\_overhang}: Optional extra sequence to add to the reverse primer.
        \item \texttt{reverse\_overhang\_name}: Optional name of an enzyme to create a matching reverse overhang.
        \item \texttt{target\_tm}: Desired melting temperature for the primers.
    \end{itemize}
    \item Returns:
    \begin{itemize}
        \item The forward primer, reverse primer, and the amplified DNA sequence (amplicon).
    \end{itemize}
\end{itemize}

\textbf{plasmid\_search:}
\begin{itemize}
    \item Purpose:
    \begin{itemize}
        \item Searches a plasmid database and returns the best matches based on features or plasmid names.
    \end{itemize}
    \item Parameters:
    \begin{itemize}
        \item \texttt{query}: Search term for plasmid or feature, allowing negation (using a minus sign) and logical operators (AND/OR).
    \end{itemize}
    \item Returns:
    \begin{itemize}
        \item A list of plasmids or features that match the query.
    \end{itemize}
\end{itemize}


\textbf{simulate\_pcr:}
\begin{itemize}
    \item Purpose:
    \begin{itemize}
        \item Runs a virtual PCR to simulate DNA amplification using chosen forward and reverse primers.
    \end{itemize}
    \item Parameters:
    \begin{itemize}
        \item \texttt{sequence}: DNA sequence to amplify.
        \item \texttt{forward\_primer}: Sequence for the forward primer (5' to 3') or an enzyme name for automated selection.
        \item \texttt{reverse\_primer}: Sequence for the reverse primer (5' to 3') or an enzyme name for automated selection.
    \end{itemize}
    \item Returns:
    \begin{itemize}
        \item The amplified DNA sequence (amplicon).
    \end{itemize}
\end{itemize}

\textbf{enzyme\_cut:}
\begin{itemize}
    \item Purpose:
    \begin{itemize}
        \item Simulates the cutting of a DNA sequence with a specified restriction enzyme, producing fragments.
    \end{itemize}
    \item Parameters:
    \begin{itemize}
        \item \texttt{sequence}: DNA sequence to be cut.
        \item \texttt{enzyme}: Restriction enzyme name to use for cutting.
    \end{itemize}
    \item Returns:
    \begin{itemize}
        \item A list of DNA fragments resulting from the cut.
    \end{itemize}
\end{itemize}

\textbf{gene\_search:}
\begin{itemize}
    \item Purpose:
    \begin{itemize}
        \item Searches the NCBI nucleotide database for gene matches based on a given query.
    \end{itemize}
    \item Parameters:
    \begin{itemize}
        \item \texttt{query}: Name or keyword associated with the gene.
    \end{itemize}
    \item Returns:
    \begin{itemize}
        \item Up to 5 gene matches from the NCBI database.
    \end{itemize}
\end{itemize}

\textbf{annotate:}
\begin{itemize}
    \item Purpose:
    \begin{itemize}
        \item Adds annotations to a DNA sequence to highlight major features, such as proteins and origins of replication (ORIs).
    \end{itemize}
    \item Parameters:
    \begin{itemize}
        \item \texttt{sequence}: The DNA sequence to be annotated.
    \end{itemize}
    \item Returns:
    \begin{itemize}
        \item The DNA sequence with added annotations.
    \end{itemize}
\end{itemize}


\textbf{slice\_sequence:}
\begin{itemize}
    \item Purpose:
    \begin{itemize}
        \item Extracts a specific region of a DNA sequence for ordering from a synthesis vendor.
    \end{itemize}
    \item Parameters:
    \begin{itemize}
        \item \texttt{sequence}: DNA sequence to slice.
        \item \texttt{start\_position}: Start position for slicing.
        \item \texttt{end\_position}: End position for slicing.
    \end{itemize}
    \item Returns:
    \begin{itemize}
        \item Sliced DNA region.
    \end{itemize}
\end{itemize}

\textbf{create\_sequence:}
\begin{itemize}
    \item Purpose:
    \begin{itemize}
        \item Orders a new, custom DNA sequence from a vendor.
    \end{itemize}
    \item Parameters:
    \begin{itemize}
        \item \texttt{sequence\_spec}: Specifications for the DNA sequence.
    \end{itemize}
    \item Returns:
    \begin{itemize}
        \item Custom DNA sequence.
    \end{itemize}
\end{itemize}

\textbf{find\_sequence\_overlap:}
\begin{itemize}
    \item Purpose:
    \begin{itemize}
        \item Identifies the overlap between a primer and a DNA sequence.
    \end{itemize}
    \item Parameters:
    \begin{itemize}
        \item \texttt{sequence}: DNA sequence to search within.
        \item \texttt{primer}: Primer sequence to locate.
        \item \texttt{reverse}: Boolean indicating if reverse complement is used.
    \end{itemize}
    \item Returns:
    \begin{itemize}
        \item Start and end positions of the overlap.
    \end{itemize}
\end{itemize}

\textbf{gibson:}
\begin{itemize}
    \item Purpose:
    \begin{itemize}
        \item Simulates Gibson Assembly for a set of DNA fragments.
    \end{itemize}
    \item Parameters:
    \begin{itemize}
        \item \texttt{sequences}: DNA fragments to assemble.
    \end{itemize}
    \item Returns:
    \begin{itemize}
        \item Predicted Gibson Assembly products.
    \end{itemize}
\end{itemize}

\textbf{goldengate:}
\begin{itemize}
    \item Purpose:
    \begin{itemize}
        \item Simulates Golden Gate assembly using Type IIS restriction-ligation.
    \end{itemize}
    \item Parameters:
    \begin{itemize}
        \item \texttt{sequences}: DNA fragments to assemble.
        \item \texttt{enzyme}: Restriction enzyme for the assembly (e.g., BsaI).
    \end{itemize}
    \item Returns:
    \begin{itemize}
        \item Predicted Golden Gate assembly products.
    \end{itemize}
\end{itemize}

\textbf{optimize\_translation:}
\begin{itemize}
    \item Purpose:
    \begin{itemize}
        \item Optimizes a DNA sequence for protein expression, usually targeting E. coli.
    \end{itemize}
    \item Parameters:
    \begin{itemize}
        \item \texttt{sequence}: DNA or protein sequence to optimize.
        \item \texttt{cg\_content}: Target CG content percentage.
        \item \texttt{codon\_table}: Codon table to use (e.g., 11 for bacteria).
        \item \texttt{min\_repeat\_length}: Minimum repeat length.
    \end{itemize}
    \item Returns:
    \begin{itemize}
        \item Optimized DNA sequence.
    \end{itemize}
\end{itemize}

\textbf{find\_orfs:}
\begin{itemize}
    \item Purpose:
    \begin{itemize}
        \item Finds open reading frames (ORFs) in a DNA sequence, with options for translation.
    \end{itemize}
    \item Parameters:
    \begin{itemize}
        \item \texttt{sequence}: DNA sequence to analyze.
        \item \texttt{min\_length}: Minimum length of ORFs.
        \item \texttt{codon\_table}: Codon table for translation.
        \item \texttt{strand}: Strand to search (both, forward, or reverse).
    \end{itemize}
    \item Returns:
    \begin{itemize}
        \item List of ORFs found in the DNA sequence.
    \end{itemize}
\end{itemize}

\textbf{view\_restriction\_sites:}
\begin{itemize}
    \item Purpose:
    \begin{itemize}
        \item Identifies common restriction enzyme sites within a DNA sequence.
    \end{itemize}
    \item Parameters:
    \begin{itemize}
        \item \texttt{sequence}: DNA sequence to analyze.
    \end{itemize}
    \item Returns:
    \begin{itemize}
        \item List of recognized restriction sites.
    \end{itemize}
\end{itemize}

\textbf{view\_sequence\_stats:}
\begin{itemize}
    \item Purpose:
    \begin{itemize}
        \item Returns sequence statistics.
    \end{itemize}
    \item Parameters:
    \begin{itemize}
        \item \texttt{sequence}: DNA sequence to analyze.
    \end{itemize}
    \item Returns:
    \begin{itemize}
        \item GC content, maximum homopolymer repeat length, and sequence length.
    \end{itemize}
\end{itemize}

\textbf{view\_translation:}
\begin{itemize}
    \item Purpose:
    \begin{itemize}
        \item Translates a DNA sequence into its corresponding protein sequence.
    \end{itemize}
    \item Parameters:
    \begin{itemize}
        \item \texttt{sequence}: DNA sequence to translate.
    \end{itemize}
    \item Returns:
    \begin{itemize}
        \item Translated protein sequence.
    \end{itemize}
\end{itemize}


==> support_information/tools_gsm8k.tex <==
\subsection{GSM8K tools}

\textbf{calculator:}
\begin{itemize}
    \item Purpose:
    \begin{itemize}
        \item This function calculates the result of a given mathematical expression.
    \end{itemize}

    \item Parameters:
    \begin{itemize}
        \item \texttt{expr}: A valid Python expression that represents a mathematical calculation.
    \end{itemize}

    \item Returns:
    \begin{itemize}
        \item \texttt{result}: result of the calculation.
        \item \texttt{reward }: reward associated with successfully calling this tool.
        \item \texttt{done}: whether the episodes has ended after this tool call. Always returns False.
    \end{itemize}
\end{itemize}

\textbf{submit\_answer}
\begin{itemize}
    \item Purpose:
    \begin{itemize}
        \item This function submits a proposed answer and checks if it is correct, marking the action as terminal.
    \end{itemize}

    \item Parameters:
    \begin{itemize}
        \item \texttt{answer}: The answer proposed by the user.
    \end{itemize}

    \item Returns:
    \begin{itemize}
        \item \texttt{correct}: whether the agent's answer is correct or not.
        \item \texttt{reward}: reward associated with the given answer.
        \item \texttt{done}: whether the episodes has ended after this tool call. Always returns a positive value, indicating that after submitting an answer the episodes has ended.
    \end{itemize}
\end{itemize}


==> support_information/tools_hotpotqa.tex <==
\subsection{HotPotQA tools:}

\textbf{search:}
\begin{itemize}
    \item Purpose:
    \begin{itemize}
        \item This tool searches for a specified entity on Wikipedia and sets the Wikipedia page as the current state where lookup tools can be used.
    \end{itemize}

    \item Parameters:
    \begin{itemize}
        \item \texttt{entity} (\texttt{str}): The name of the entity to search for on Wikipedia.
    \end{itemize}

    \item Returns:
    \begin{itemize}
        \item The first paragraph of the Wikipedia page if the page is found.
    \end{itemize}
\end{itemize}

\textbf{lookup:}
\begin{itemize}
    \item Purpose:
    \begin{itemize}
        \item Finds all occurrences of a specified keyword within the current Wikipedia page.
    \end{itemize}

    \item Parameters:
    \begin{itemize}
        \item \texttt{keyword} (\texttt{str}): The keyword to search for within the page’s sentences.
    \end{itemize}

    \item Returns:
    \begin{itemize}
        \item The \texttt{n}th paragraph in the current Wikipedia page where the keyword appears, where \texttt{n} is the number of consecutive times this tool has been called with the same keyword.
    \end{itemize}
\end{itemize}

\textbf{submit\_answer:}
\begin{itemize}
    \item Purpose:
    \begin{itemize}
        \item Completes the task by submitting a final answer to the question.
    \end{itemize}

    \item Parameters:
    \begin{itemize}
        \item \texttt{answer} (\texttt{str}): The answer to submit.
    \end{itemize}

    \item Returns:
    \begin{itemize}
        \item A message indicating that the episode has finished.
    \end{itemize}
\end{itemize}


